Boundary Discretization and Reliable Classification Network for Temporal Action Detection

Temporal action detection aims to recognize the action category and determine each action instance's starting and ending time in untrimmed videos. The mixed methods have achieved remarkable performance by seamlessly merging anchor-based and anchor-free approaches. Nonetheless, there are still two crucial issues within the mixed framework: (1) Brute-force merging and handcrafted anchor design hinder the substantial potential and practicality of the mixed methods. (2) Within-category predictions show a significant abundance of false positives. In this paper, we propose a novel Boundary Discretization and Reliable Classification Network (BDRC-Net) that addresses the issues above by introducing boundary discretization and reliable classification modules. Specifically, the boundary discretization module (BDM) elegantly merges anchor-based and anchor-free approaches in the form of boundary discretization, eliminating the need for the traditional handcrafted anchor design. Furthermore, the reliable classification module (RCM) predicts reliable global action categories to reduce false positives. Extensive experiments conducted on different benchmarks demonstrate that our proposed method achieves competitive detection performance. The code will be released at https://github.com/zhenyingfang/BDRC-Net.

==> tabs/a2net_cmp_bdrc.tex <==
\begin{tabular}{c|ccccc|c}
\hline
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{mAP@tIoU(\%)} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}average mAP(\%)\\ $[0.5:0.1:0.9]$\end{tabular}} \\
                        & 0.5   & 0.6   & 0.7  & 0.8  & 0.9 &                                                                  \\ \hline \hline
A2Net                   & 45.5  & 32.5  & 17.2 & -    & -   & -                                                          \\
A2Net$^\dagger$         & 45.2  & 32.6  & 19.1 & 6.9  & 0.9 & 21.4                                                           \\
BDRC-Net w/o RCM        & 46.9  & 35.9  & 23.9 & 10.9 & \textcolor{red}{1.8} & 23.9                                                              \\
BDRC-Net                & \textcolor{red}{49.8}  & \textcolor{red}{37.8}  & \textcolor{red}{25.0} & \textcolor{red}{11.3} & \textcolor{red}{1.8} & \textcolor{red}{25.1}   \\ \hline
\end{tabular}

==> tabs/complexity.tex <==
\begin{tabular}{c|ccc}
\hline
Method & A2Net & \begin{tabular}[c]{@{}c@{}}BDRC-Net\\ w/o RCM\end{tabular} & BDRC-Net \\ \hline \hline
Infe. Time / ms & 7.6 & 7.5 & 7.7 \\
FLOPs / G & 1.24 & 1.20 & 1.24 \\ \hline
\begin{tabular}[c]{@{}c@{}}average mAP(\%)\\ $[0.5:0.1:0.9]$\end{tabular} & 20.9 & 24.1 & 25.7 \\ \hline
\end{tabular}

==> tabs/lambda_norm.tex <==
\begin{tabular}{c|ccc|c}
\hline
\multirow{2}{*}{$\lambda_{norm}$} & \multicolumn{3}{c|}{mAP@tIoU(\%)} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}average mAP(\%)\\ $[0.5:0.1:0.9]$\end{tabular}} \\
 & 0.5 & 0.7 & 0.9 &  \\ \hline
80 & 47.7 & 24.8 & 1.8 & 24.4 \\
90 & 50.6 & 25.2 & 2.0 & 25.7 \\
100 & 50.4 & 24.9 & 1.8 & 25.5 \\ \hline
\end{tabular}

==> tabs/lambda_rs.tex <==
\begin{tabular}{c|ccc|c}
\hline
\multirow{2}{*}{$\lambda_{rs}$} & \multicolumn{3}{c|}{mAP@tIoU(\%)} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}average mAP(\%)\\ $[0.5:0.1:0.9]$\end{tabular}} \\
 & 0.5 & 0.7 & 0.9 &  \\ \hline \hline
0.4 & 49.6 & 25.3 & 1.9 & 25.4 \\
0.5 & 50.6 & 25.2 & 2.0 & 25.7 \\
0.6 & 48.0 & 25.0 & 2.0 & 24.9 \\
0.7 & 46.1 & 21.8 & 1.3 & 22.9 \\ \hline
\end{tabular}
